Linear Strands of Initial Ideals of Determinantal Facet Ideals

A determinantal facet ideal (DFI) is an ideal $J_\Delta$ generated by maximal minors of a generic matrix parametrized by an associated simplicial complex $\Delta$. In this paper, we construct an explicit linear strand for the initial ideal with respect to any diagonal term order $<$ of an arbitrary DFI. In particular, we show that if $\Delta$ has no \emph{1-nonfaces}, then the Betti numbers of the linear strand of $J_\Delta$ and its initial ideal coincide. We apply this result to prove a conjecture of Ene, Herzog, and Hibi on Betti numbers of closed binomial edge ideals in the case that the associated graph has at most $2$ maximal cliques. More generally, we show that the linear strand of the initial ideal (with respect to $<$) of \emph{any} DFI is supported on a polyhedral cell complex obtained as an induced subcomplex of the \emph{complex of boxes}, introduced by Nagel and Reiner.

==> figures/graph.tex <==
\begin{figure}[h]
\begin{tikzpicture}[scale=0.4]
\filldraw[thick] 
(0,0) circle (4pt) --
(5,0) circle (4pt)  -- 
(5,5) circle (4pt) --
(0,5) circle (4pt) --
(0,0);
\filldraw[thick] (5,5)--(7.5, 2.5) circle (4pt) -- (5,0);
\draw[thick] (0,0)--(5,5);
\draw[thick] (0,5)--(5,0);
\node at (-0,-0.75) {$2$};
\node at (5,-0.75) {$4$};
\node at (5,5.75) {$3$};
\node at (-0,5.75) {$1$};
\node at (8, 2.5) {$5$};
\end{tikzpicture}
\caption{A graph with two maximal cliques given by vertex sets $\{1,2,3,4\}$ and $\{3,4,5\}$.}\label{fig: BEI2cliques}
\end{figure}
